Adversarial training approach for local data debiasing

The widespread use of automated decision processes in many areas of our society raises serious ethical issues concerning the fairness of the process and the possible resulting discriminations. In this work, we propose a novel approach called GANsan whose objective is to prevent the possibility of any discrimination i.e., direct and indirect) based on a sensitive attribute by removing the attribute itself as well as the existing correlations with the remaining attributes. Our sanitization algorithm GANsan is partially inspired by the powerful framework of generative adversarial networks (in particular the Cycle-GANs), which offers a flexible way to learn a distribution empirically or to translate between two different distributions. In contrast to prior work, one of the strengths of our approach is that the sanitization is performed in the same space as the original data by only modifying the other attributes as little as possible and thus preserving the interpretability of the sanitized data. As a consequence, once the sanitizer is trained, it can be applied to new data, such as for instance, locally by an individual on his profile before releasing it. Finally, experiments on a real dataset demonstrate the effectiveness of the proposed approach as well as the achievable trade-off between fairness and utility.

==> 06-GenerativeAdversarialNetwork.tex <==
\subsection{Generative adversarial network}
\label{sec:gan}

\emph{Generative Adversarial Network} (GAN) is an approach in machine learning introduced to solve the difficult problem of modelling and learning high dimensional distributions (\emph{e.g.}, pictures).
Typically, in a GAN, two neural networks compete against each other in a zero-sum game framework~\cite{GanIan2014}.
The first neural network, hereafter referred to as the \emph{generator} $G$, aims to learn to generate from noise $P_z$ data close enough to a given distribution $P_{data}$, its production being the final objective of the GAN.
The second neural network, hereafter referred to as the \emph{discriminator} $D$, learns to discriminate whether a given sample originates from the generator or from the training data. 

Despite its intuitive aspect and the fact that GANs are powerful tools for modelling distributions, training a GAN can be difficult and often require important engineering efforts for ensuring its success~\cite{zhu2017unpaired}.
For instance, during the training phase, if the discriminator (respectively the generator) outperforms its counterpart by a large margin, the later will not be able to catch-up and improve its performance. 

Mirza and Osindero have proposed an extension of GAN, called \textsf{CycleGAN} \cite{mirza2014conditional}, in which the goal is to learn to translate between two  distributions. 
Our approach, \gansan{}, is inspired by the framework of GANs and CycleGANs in the sense that our objective is to learn to remove the dependency between the sensitive attribute and the other attributes without having an explicit description of these dependencies and by solely relying on the ability of an adversary to distinguish (or not) between the sensitive and default groups.




==> GanFramework.tex <==
\begin{figure}
    \centering
    \resizebox{.6\linewidth}{!}{
        \begin{tikzpicture}[node distance=2cm, every node/.style={fill=white, font=\sffamily}, align=center]
            \node (randD)            [noiseNodes, xshift=-2.5cm] {Noise / Random Input: $P_{z}$};
            \node (realD)            [originals, xshift=2.5cm] {Real Data: $P_{data}$};
            \node (generator)        [sanitizerNode, below of=randD] {Generator Network, $G(z)$};
            %\node (oGenerated)       [process, below of=sanitizer] {Sanitized Set};
            \node (disc)             [discriminatorNode, below of=generator, xshift=2.5cm] {Discriminator Network $D(x)$};
            \node (d_output)         [process, below of=disc] {$True$ or $False$};
            
            \draw[->]              (realD) -- node[text width=2cm]
                                           {original data}
                                           (disc);
            \draw[->]              (randD) -- (generator);
            \draw[->]              (generator) -- (disc);
            \draw[->]              (disc) -- (d_output);
            \draw[->]              (d_output) -| (generator);
        \end{tikzpicture}
        }w
    \caption{Overview of the GAN framework. The generator $G(z)$ takes input from a noise distribution $Z$ and guided by the discriminator $D(x)$, generates new data matching the prior distribution. The discriminator $D(x)$ is trained to differentiate real data from the fake ones produced by the generator by taking as input samples from both distributions.}
    \label{fig:GanProcess}
\end{figure}
